Uncertainty-aware Knowledge Tracing

Knowledge Tracing (KT) is crucial in education assessment, which focuses on depicting students' learning states and assessing students' mastery of subjects. With the rise of modern online learning platforms, particularly massive open online courses (MOOCs), an abundance of interaction data has greatly advanced the development of the KT technology. Previous research commonly adopts deterministic representation to capture students' knowledge states, which neglects the uncertainty during student interactions and thus fails to model the true knowledge state in learning process. In light of this, we propose an Uncertainty-Aware Knowledge Tracing model (UKT) which employs stochastic distribution embeddings to represent the uncertainty in student interactions, with a Wasserstein self-attention mechanism designed to capture the transition of state distribution in student learning behaviors. Additionally, we introduce the aleatory uncertainty-aware contrastive learning loss, which strengthens the model's robustness towards different types of uncertainties. Extensive experiments on six real-world datasets demonstrate that UKT not only significantly surpasses existing deep learning-based models in KT prediction, but also shows unique advantages in handling the uncertainty of student interactions.

==> problem.tex <==
% In this study, our core task focuses on leveraging students' past interaction histories to accurately predict the probability that 
% they will correctly answer any given question \( q^* \).
For each student \( S \), we assume that we have a series of \( T \) interactions arranged in chronological order, i.e., \( S = \{s_j\}_{j=1}^{T} \). Each interaction can be represented as a structured quadruple \( s = \langle q, \{c\}, r, s \rangle \), where \( q \) is the specific question, \( \{c\} \) is the set of knowledge components associated with the question, \( r \) is the binary student response (correct or incorrect), and \( s \) is the time point at which the student answered. Our ultimate goal is to construct a model based on this information to evaluate and predict the probability \( \hat{r}^* \) that a student will answer correctly to a given question \( q^* \).


% This requires the model to capture the dynamic changes in the student's learning trajectory
% To achieve this, the key is to capture the dynamic changes in students' learning trajectory.
% and to understand the intrinsic relationship between the mastery of knowledge components and problem-solving abilities.%这句话可能会引入更复杂的debate。


==> uncertainty.tex <==
Uncertainty, as an inherent unpredictable component in model predictions or outcomes, plays a crucial role in supporting societal decision-making, quantitative research, and machine learning applications \cite{Helton2008, wimmer2023quantifying, gal2016uncertainty}. The prerequisite for delving into these uncertainties consist of establishing the foundation for building user trust in the system and enhancing the model reliability \cite{Sanchez2022}. To further refine this concept, uncertainty can be divided into two main categories: epistemic uncertainty and aleatory uncertainty \cite{gal2016uncertainty, hullermeier2021aleatoric}.

\textbf{Epistemic uncertainty} arises from a lack of knowledge about the system or process and can be reduced by acquiring more information or improving the model, involving an incomplete understanding of certain parameters or system behaviors\cite{Chen2020}. In knowledge tracing, epistemic uncertainty originates from the diversity in students' learning abilities and knowledge absorption levels and arises from varying depths of students' understanding of concepts so that is hard to capture. This uncertainty relates to each student's unique learning path, comprehension skills, and learning strategies. Even when faced with the same learning materials and environment, different students may exhibit significant differences in knowledge mastery and application, leading to variations in learning outcomes and complexity in assessing students' knowledge levels.


\textbf{Aleatory uncertainty} is inherent in the data itself, stemming from the randomness in the data generation process. This type of uncertainty cannot be reduced by collecting more data \cite{hullermeier2021aleatoric}. Examples include measurement noise, inherent variability in the data, and randomness in the environment. In the field of knowledge tracing, this uncertainty might manifest as students making careless mistakes or guessing on questions.

By understanding and quantifying these two types of uncertainty, we can build models that are both accurate and trustworthy \cite{abdar2021review}. We have carefully designed our KT model to effectively tackle both epistemic and aleatory uncertainty.
